Database Queries that Explain their Work

Provenance for database queries or scientific workflows is often motivated as providing explanation, increasing understanding of the underlying data sources and processes used to compute the query, and reproducibility, the capability to recompute the results on different inputs, possibly specialized to a part of the output. Many provenance systems claim to provide such capabilities; however, most lack formal definitions or guarantees of these properties, while others provide formal guarantees only for relatively limited classes of changes. Building on recent work on provenance traces and slicing for functional programming languages, we introduce a detailed tracing model of provenance for multiset-valued Nested Relational Calculus, define trace slicing algorithms that extract subtraces needed to explain or recompute specific parts of the output, and define query slicing and differencing techniques that support explanation. We state and prove correctness properties for these techniques and present a proof-of-concept implementation in Haskell.

==> TODO.tex <==
\section{TODO}

\paragraph{Intro.}  Incorporate these into the introduction. 

\begin{enumerate}
\item  Slices need to make sense.  they are runnable. 

\item the guiding principle: invert a derivation step guided by the
  part of the result that we are interested in . 

\item Slice?  How can we compute it?   Of course we do not want to
  generate many labels. 

\item How to deal with substitution.  Substitution and slicing
  compete.  Substitution creates sharing.  For slicing we want to
  specialize as much as possible. 

  There may be non-compositional ways of generating slices.   
\end{enumerate}




\begin{description}

\item[Forward Slicing:]  Work forward slicing out.  Backward and
  forward can be used in  combination.  For example, you can do a
  backward slice first and the ask if this label contributes to the
  backward slice and in what way, which can be answered by taking a
  forward slice.  When taking a forward slice, types matter, because a
  pair will always be a pair so the path to the result will, for
  example, be always well defined. 
  

\item[Major issue (June 18, Umut): DONE (June 19)] 

Consider the example, let x = (1,2) in (snd x, fst x) end\\

The current slicing rules don't deal with this (i.e., multiple use of
the same derivation).  One approach is to subtitute $T_1$ into the
hole and then slice on.

$\bullet$ To solve this issue, we substitute trace during a
slice/let.

\item[Labeled vs unlabled values (June 18, Umut). DONE (June 19):]
  Labeled vs unlabeled value, when are they ``touched''.  Consider the
      following example (assuming a, b, c are label),

let x = (1a,2b)c in (fst x, snd x, x, fst x + 4)

When do you touch 2b when performing the addition...  The judgements
need to be careful with this issue.  Right now, they are sloppy. 

The key point  here is to note that any value will be
``downward-closed'' once a value is a labeled all its descendants will
    also be.

$\bullet$ The idea is to touch all labels when we see them.  An
    expression with a label is not a value, so we just touch it when
    we see it by recording it in the trace.  Paths guide us to the
    right places.

\item[Labeling of the input expression (June 18, Umut). Partially
  DONE.] I think we can label whatever parts of the subexpression that
  we would like and adjust the slicing to mind all the labels
  accordingly.  For multisets, we will need to label the sets
  themselves as well, i.e., we will label *all* values.

  Now the cool thing is that labeling all values will probably be
  sufficient for most kinds of provenance.  But we can do more, we can
  label any other part of the expressions.  Then we would have
  provenance information relating the parts of the query to the
  result, so that we can ask the question of what part of the result
  would be effected if I change some part of the query.  For this, we
  would probably formulate a "forward" slicing technique.  {\bf I
    think that this should be a separate section.} Kinda like here is
  the good old stuff but now check out this cool move.

   This reminds me the slicing approach that in the paper is
   ``backwards''.  It takes a path into the result and finds the slice
       that computes that path.  We probably want to do the reverse as
       well.

$\bullet$ The idea here is to just allow expression to have labels
       arbitrarily and touch the labels when we see them during
       evaluation.  We still need to think about what it means to do a
       forward slice and all that. 

\item[When to generate labels (June 18, Umut). DONE.:] We need labels
  because of the variable binding.  I feel that it would be helpful to
  separate input labels from these on-the-fly labels, because they are
  purely used to guide substitution.  So let's put these aside for a
  second.  May be we would call them "tags" or "guides" or "locations"
  or some such thing but not "labels" .

  Now I conjecture that we don't need to create any more labels at
  all.  In particular, the run-time values that we generate never need
  to be labeled.  In fact, once I touch a labeled value (e.g., $2^l$
  from input expression), I can strip off its label and return the
  unlabeled value instead.

For example, the rule to evaluate $n^l$ would be

$n^l \red n, < l >_n$

Note that the trace records the label.  The returned result is not
labeled anymore.

The reason for why I feel that this will work is the "grand idea" that
paths suffice to navigate traces/derivations leading us to the right
place.  In particular, guided by a path, we will locate in the trace
all evaluation of subexpressions of the input expression that
contribute to the output.  Now the trace will record labels (as above)
for all such use of input labels and we will be able to identify all
dependences.

$\bullet$ No need to generate labels except at a let.  There is no
need to separate guides from conventional labels on vales.  It works
just fine.  

\end{description}


==> dependency.tex <==
\newcommand{\pow}{\mathcal{P}}
\newcommand{\eval}[3]{#1 , #2 \Downarrow #3}
\newcommand{\sqleq}{\sqsubseteq}
\newcommand{\meet}{\sqcap}
\newcommand{\eq}{\stackrel{{\tiny \times}}{\approx}}

\section{Dependency provenance}

\begin{definition}
  [Sets with locations] Consider a set of locations $L$.  A \emph{set
    with locations} is a structure $(X,lab: X \to \pow(L),\eq :
  \pow(L) \to \pow(X \times X))$.  We write $x\eq_L x'$ instead of
  $(x,x') \in \eq(L)$.  A set with locations must satisfy the
  following properties:
  \begin{eqnarray*}
    \forall x,x'.~ x \eq_\emptyset x' &\iff& x = x'\\
    \forall x,x'.~x \eq_{locs(x)} x' \\
    \forall L,L',x,x'.~ L \subseteq L' \wedge  x \eq_L x' &\Rightarrow& x \eq_{L'} x'\\
    \forall L,L',x,x'.~x \eq_L x' \wedge x \eq_{L'} x' &\Rightarrow& x \eq_{L \cap L'} x'
  \end{eqnarray*}
\end{definition}

Consider values adorned with locations.  (This means that each part of
the value has a path, identifier or some other way of ``pointing'' to
that part - for now, we leave the particular mechanism for
``pointing'' unspecified).  We only require that there is a notion of
equality on such values ``indexed'' by locations (or sets of
locations.  Specifically, we say that $v =_l v'$ to indicate that $v$
and $v'$ are equal ``except for'' location $l$, and similarly $v =_L
v'$ to indicate that $v$ and $v'$ are equal ``except for'' locations
in $L$.  We also assume that there is a reachability relation on
locations: namely, $l \leadsto_v l'$ means that $l'$ is reachable from
$l$.  This is assumed to be compatible with equality as follows: $v
=_{l'} v'$ and $l \leadsto^v l'$ implies $v =_l v'$.  Finally, we
define a function $C_v : loc(x) \to \pow(loc(x))$ as follows: $C_v =
\{l' \mid l \leadsto^v l'\}$.

Now consider a function $f : X \to Y$ on such values.  For example, we
can take a standard a operational semantics $\eval{\gamma}{e}{v}$ that
evaluates an expression $e$ on a variable environment $\gamma$ to a
value $v$ as a baseline, and extend it to a semantics that operates on
values with locations.  (Technically, this is not a function but a
relation, since locations generation may be nondeterministic, but it
is a function if we ignore the locations).

We want to define a notion of ``provenance'' as a relation between the
input and output locations, subject to certain semantic conditions.
Let $y = f(x)$, and consider $l \in loc(x)$ and $L \subseteq loc(y)$.
Then we say that $L$ captures all dependences of $l$ if for any $x'
=_l x$ we have $f(x') =_L f(x)$.  Moreover, a function $F :loc(x) \to
loc(y)$ is dependency correct provided that $F(l)$ captures all
dependences of $l$ for each $l \in loc(x)$.  Equivalently, we can
speak about a relation $R \subseteq loc(x) \times loc(y)$, which can
obviously be obtained from $F$ and vice versa.

Dependency-correctness does not uniquely determine the function $F$ or
relation $R$.  In particular, the total relation $R = loc(x) \times
loc(y)$ is always dependency-correct for any $f,x,y$.  Hence, we also
introduce a notion of a dependency-correct $F$ being \emph{more
  accurate} or \emph{more informative} than another $F'$.  Our goal is
to identify a relation $\sqleq$ that is both intuitively appealing and
possesses good theoretical properties, i.e. it is a semilattice with
unique ``most accurate'' dependency-correct elements.  (This will turn
out to be a quasi-order but we can get a partial order with unique
extrema true only up to an appropriate equivalence relation).

\paragraph{Comparing dependency maps}
We will consider first a syntactic definitions that seem informally
well-motivated ways of capturing the idea that one dependency map is
more informative than another.  We first consider an order that does
not have unique extrema.
%
\[F \sqleq_0 G \iff \forall l \in loc(v). F(l) \subseteq G(l)\]
%
To see why this deos not work, consider [EXAMPLE from notes].  We have
three dependency maps $F,G,H$ that are mutually incomparable using
this order, but $F$ and $G$ both seem ``less informative'' than $H$.

In avoid this problem, we refine the above definition.


We will show that with this definition, $\sqleq$ is a quasiorder:
\begin{proposition}
  $\sqleq$ is reflexive and transitive, but not antisymmetric
\end{proposition}
\begin{proof}
  Reflexivity and transitivity are straightforward.  An example of
  antisymmetry is to take $x = l_o$, $y = l_1 \to l_2$, $F_1 =
  \{(l_0,l_1)\}$ and $F_2 = \{(l_0,l_1),(L_0,l_2)\}$.  It is easy to
  see that $F_1 \sqleq F_2$ and conversely $F_2 \sqleq F_1$, but they
  are not equal.
\end{proof}

\begin{figure}
  \centering
%  \includegraphics{closure.pdf}
  \caption{Counterexample to antisymmetry}
\end{figure}
We write $F_1 \equiv F_2$ to indicate $F_1 \sqleq F_2$ and $F_2 \sqleq
F_1$.

Recall that locations are naturally ordered by the structure of teh
value tree; we write $l \leadsto^x l'$ to indicate that $l$ precedes
$l'$ along a path from the root.  It is useful to work in terms of
sets of locations closed under $\leadsto^x$.  We define the closure
$C_x : loc(x) \to \pow(loc(x))$ as follows:
%
\[C_x(l) = \{l' \mid l \leadsto^x l'\}\]
%
We overload notation to lift closure to sets of locations by writing
$C_x[L] = \bigcup\{C_x(l) \mid l \in L\}$.  Moreover, we say that a
dependency map $F$ is \emph{closed} if $C_y \circ F = F$.  The closure
operator has the following nice properties:
\begin{proposition}
  $C_x$ is a (formal) closure operator acting on sets of locations:
  \begin{eqnarray}
    L &\subseteq& C_x[L]\\
    L \subseteq C_x[L'] & \Rightarrow & C_x[L] \subseteq C_x[L']\\
    C_x(L) &=& C_x[C_x[L]]
  \end{eqnarray}
  Similar properties hold for $C_v$ acting on dependency maps by left
  composition.
\end{proposition}
\begin{proof}
  It is srtaightforward to verify that $C_x$ is a closure operator on
  sets of locations.  For dependency maps, the desired properties lift
  in the obvious way.
\end{proof}

We can also show that closed dependency maps are well-behaved with
respect to the information ordering:
\begin{proposition}
  \begin{eqnarray}
    F \sqleq G &\iff& F \subseteq C_y \circ G\\
    F \equiv G &\iff& C_y\circ F = C_y \circ G\\
    F &\equiv& C_y(F)
  \end{eqnarray}
\end{proposition}
\begin{proof}
  For the first part, if $F \sqleq G$ then we want to show that $F
  \subseteq C_y(G)$.  Let $l$ be given and consider $l' \in F(l)$.
  Since $F \sqleq G$ there must exist a $l'' \in G(l)$ such that $l''
  \leadsto^y l'$, hence by definition $l \in C_y(G(l))$.  This shows
  that $F \subseteq C_y \circ G$, as desired.  Conversely, suppose
  $C_y \circ F \subseteq C_y \circ G$.  Let $l \in loc(x)$ and $l' \in
  F(l)$ be given.  We wish to find an $l''$ in $G(l)$ such that $l''
  \leadsto^y l'$.  Note that $F(l) \subseteq C_y(G(l))$ so $l' \in
  C_y(G(l))$.  Hence there exists $l'' \in G(l)$ such that $l''
  \leadsto^y l'$, as desired.

  For the second part, note that $F \equiv G$ is equivalent to
%
  \[F \subseteq C_v(G) \wedge G \subseteq C_y(F)\]
%
  by the first part.  Then
%
  \[C_y(F) \subseteq C_y(C_y(G)) \wedge C_y(G) \subseteq C_y(C_y(F))\]
%
  Hence
%
  \[C_y(F) \subseteq C_y(G) \wedge C_y(G) \subseteq C_y(F)\]

  Finally, the third part follows immediately because $C_y \circ F =
  C_y \circ C_y \circ F$, using the second part.
\end{proof}

So, to simplify matters, from now on we restrict attention to closed
dependency maps.  (Such maps may have a lot of ``redundant'' edges,
but we can always represent these more efficiently by pruning).

Since the set of (closed) dependency maps on a given $x,y$ is finite,
we know that \emph{minimal} elements must exist.  We ultimately want
to show that for any finite set of dependency maps has a unique
(closed) greatest lower bound.  Accordingly, given $F,G$, we define an
operation $F \meet G$ as follows:
%
\[(F \sqcap G)(l) = C_y(F(l)) \cap C_y(G(l))\]
%
We wish to show that this is a greatest lower bound operator making
the set of closed dependency maps into a lattice.
\begin{proposition}
  For any $F,G$, we have $F \meet G \sqleq F$ and $F \meet G \sqleq
  G$.  Moreover, if $H \sqleq F$ and $H \sqleq G$ then $H \sqleq F
  \meet G$.
\end{proposition}
\begin{proof}
  For the first part, we show that $F \meet G \sqleq F$ (the other
  part is symmetric).  It suffices to show that $F \meet G \subseteq
  C_y(F)$.  Let $l$ be given.  Then
%
  \[(F \meet G)(l) = C_y(F(l)) \cap C_y(G(l)) \subseteq C_y(F)\]
% 
  so we are done.

  For the second part, let $H \sqleq F$ and $H \sqleq G$ be a lower
  bound.  Then $H \subseteq C_y(F)$ and $H \subseteq C_y(G)$ so $H
  \subseteq C_y(F) \cap C_y(G) = F \meet G$.
\end{proof}

This shows that the set of (closed) dependency maps is a lower
semilattice, and since it is also finite, it is necessarily complete
(any set of closed dependency maps has a greatest lower bound).

Finally, we will show that the meet operation preserves dependency-correctness.  To do this we first need some basic properties:
\begin{proposition}
  \begin{itemize}
  \item $L \subseteq L'$ and $x \eq_L x'$ implies $x \eq_{L'} x'$.  In
    particular, $x \eq_L x'$ implies $x\eq_{C_x(L)} x'$.
  \item Assume $L,L'$ are closed (as subsets of $loc(x)$).  If $x \eq_L
    x'$ and $x\eq_{L'}x'$ then $x\eq_{L \cap L'} x'$.
  \item  $F \in DC(f,x,y)$ iff $C_y \circ F \in DC(f,x,y)$.
  \end{itemize}
\end{proposition}
\begin{theorem}
  If $F,G \in DC(f,x,y)$ then $F \meet G \in DC(f,x,y)$.
\end{theorem}
\begin{proof}
  Without loss of generality (by part 3 above) consider only closed
  dependency maps $F,G$.  Then set $H = F \meet G$; observe that $H$
  is closed and $H \sqleq F,G$.  We want to show that $H \in
  DC(f,x,y)$.  Let $l \in loc(x)$ and $x'$ with $x \eq_l x'$ be given;
  we want to conclude that $y \eq_{H(l)} y'$.  Now by assumption we know
  that $y\eq_{F(l)} y'$ and $y\eq_{G(l)} y'$.  Moreover, both $F$ and $G$
  are closed by assumption so we have $y \eq_{F(l) \cap G(l)} y'$.
  Moreover, clearly $H(l) = C_y(F(l)) \cap C_v(G(l)) = F(l) \cap
  G(l)$, so we can conclude $y = {H(l)} y'$.
\end{proof}


\paragraph{Semantic interpretation of $\sqleq$}

Let's now try to formalize the idea that $F$ and $G$ are ``less
informative'' than $H$.  We can interpret a dependency map in (at
least) two ways.

Recall that $F$ being dependency-correct for
$(f,x,y)$ means that we must be able to make predictions about the
behavior of $f$ under changes to $x$.  Thus, given $F$ we can define a
relation 
%
\[\hat{F} = \bigcup_{l \in loc(x)}\{(x',y') \mid x \eq_l x'
\text{ and } y \eq_{F(l)} y'\}.\]
%
Clearly, if $F$ is dependency-correct with respect to $f$ then $f
\subseteq F$.  We call $\hat{F}$ the \emph{information content} of $F$.
Now recalling $F,G,H$ in the example above, we have that $\hat{F}
\supseteq \hat{H} \subseteq \hat{G}$.  This is because any change we
can make at a leaf can be simulated by making a change further up the
tree.

\begin{proposition}
  $F_1 \sqleq F_2$ implies $\hat{F_1} \subseteq \hat{F_2}$.
\end{proposition}
\begin{proof}
  If $F_1 \sqleq F_2$ then suppose $(x,y) \in \hat{F_1}$.
\end{proof}

The second possible interpretation of a dependency map is as a set of
functions (satisfying $f(x) = y$) with respect to which it is
dependency correct:
%
\[\bar{F} = \{f : X \to Y \mid f(x) = y, \text{$F$ dependency correct wrt f}\}\]
%
Similar to the above, we can define an information ordering $\bar{F}
\subseteq \bar{G}$ which says that $F$ is more informative than $G$ provided that fewer functions are consistent with it.

Obviously, we have $f \in \bar{F}$ iff $F \in DC(f,x,y)$.

\begin{proposition}
  $\hat{F} \subseteq \hat{G}$ implies $\bar{F} \subseteq \bar{G}$.
\end{proposition}
\begin{proof}
  Assume $\hat{F} \subseteq \hat{G}$.  Let $f \in \bar{F}$ be given.
  Then $f(x) = y$ and $F \in DC(f,x,y)$.  We want to show that $f \in
  \bar{G}$ also.  Obviously, $f(x) = y$, so we just need to show that
  $G \in DC(f,x,y)$.  Now suppose $l \in locs(x)$ and $x'$ such that
  $x \eq_l x'$ are given.  Since $F$ is dependency-correct for $f$, we
  have $y \eq_{F(l)} f(x')$.  Moreover, since both $x \eq_l x'$ and $y
  \eq_{F(l)} f(x')$ hold, we have $(x',f(x')) \in \hat{F} \subseteq
  \hat{G}$.  Unpacking the definition of $\hat{G}$, we can conclude
  that $y \eq_{G(l)} f(x')$, as desired.  Hence $G$ is
  dependency-correct for $F$, so $f \in \bar{G}$ and $\bar{F}
  \subseteq \bar{G}$.
\end{proof}

\textbf{Open problem:} Resolve the relationships between ``syntactic''
accuracy $\sqleq$ and the two ``semantic'' orderings based on
$\hat{F}$ and $\bar{F}$.  Are the implications proved above strict?
Or are all three orderings equivalent?



==> fig-example-if-1-0.tex <==
\sethlcolor{SpringGreen}
\begin{figure}
\small
\fbox{\parbox{\columnwidth}{
\[
\begin{array}{c}
\inferrule*
{
      \inferrule*{
        \inferrule*
        {
          \inferrule*
          {
            \hlm{a \red a} \\ b \red b
          }
          {
            \kwpair{a}{b} \red \kwpair{a}{b}
          }             
        }
        {
          \kwfst{\kwpair{a}{b}} \red a
        }
        \\
        \inferrule*{\strut}{\hlm{1 \red 1}}
        \\
        \hlm{(a=1)}
     }
    {
      \hlm{\kwfst{\kwpair{a}{b}} = 1     \red \kwtrue}
    }
    \\
    \inferrule*
    {
      \strut
    }
    {
      \hlm{0 \red 0}
    }
}
{
  \hlm{
  \kwif{\kwfst{\kwpair{a}{b}} = 1}{0}{1}
  \red
  0}
}
\end{array}
\]
}}

\nocaptionrule

\caption{The slice for conditionals includes the expression for the
skipped branch.}  
\label{fig:example-if-1-0}
\end{figure}



==> fig-example-if-fst-1-then-0-else-1.tex <==
\sethlcolor{SpringGreen}
\begin{figure}
\small
\fbox{\parbox{\columnwidth}{
\[
\begin{array}{c}
\inferrule*
{
\begin{array}{c}
\parbox[b]{1.1in}{
\[
  \inferrule*
  {
    \inferrule*
    {
      \hlm{1 \red 1}
      \\
      {2 \red 2}
    }
    {
      \kwpair{1}{2}
      \red 
      \kwpair{1}{2}
      }
  }
  {
    \kwpair{1}{2}
    \red 
    \kwpair{1}{2}
  }
\]
}
%  \\
\parbox[b]{2in}{
\[
  \inferrule
  {
   \inferrule{
      \inferrule*
      {
       \kwpair{1}{2} \red \kwpair{1}{2}
      }
      {
        \kwfst{\kwpair{1}{2}}
        \red
        1
      }
      \\
      (1 = 1)
    }
    {
    \hlm{\kwfst{\kwpair{1}{2}} = 1     \red \kwtrue}
    }
    \\
    \inferrule
    {
    \strut
    }
    {
    \hlm{0 \red 0}
    }
  }
  {
   \hlm{\kwif{\kwfst{\kwpair{1}{2}} = 1}{0}{1} \red  0}
  }
\]
}
\end{array}
}
{
\kwlet
{x}
{\bindl{c}{\kwpair{\bindl{a}{1}}{\bindl{b}{2}}}}
{\kwif{\kwfst{x} = 1}{0}{1}}
\red
0
}
\end{array}
\]
}}

\nocaptionrule
\caption{A derivation and a slice (highlighted).}
\end{figure}



==> fig-example-let-if.tex <==
\sethlcolor{SpringGreen}
\begin{figure}
\small
\fbox{\parbox{\columnwidth}{
\[
\begin{array}{c}
\inferrule*
{
  \inferrule*
  {
   \dctx^{e_1}
  }
  {
    e_1
    \red 
    (\hlm{v_1},v_2)
  }
  \\
  \inferrule*
  {
    \inferrule*
    {
      \hlm{\dctx^{e_2}}
    }
    {
      \hlm{e_2 \red \kwtrue}
    }
    \\
    \inferrule*
    {
     \strut
    }
    {
      \kwfst{\kwpair{v_1}{v_2}}
      \red
      v_1
    }
  }
  {
    \hlm{
      \kwif{e_2}{\kwfst{\kwpair{v_1}{v_2}}}{\kwsnd{\kwpair{v_1}{v_2}}}
      \red
      v_1
    }
  }    
}
{
\kwlet
{x}
{e_1}
{\kwif{e_2}{\kwfst{x}}{\kwsnd{x}}}
\red
\hlm{v_1}
}
\end{array}
\]
}}

\nocaptionrule
\caption{Each use of a variable can require a different slice.}
\label{fig:example-let-if}
\end{figure}


==> fig-example-let-sum.tex <==
\sethlcolor{SpringGreen}
\begin{figure}
\small
\fbox{\parbox{\columnwidth}{
\[
\begin{array}{c}
\inferrule*
{
  \inferrule*
  {
   \dctx
  }
  {
    e
    \red 
    (v_1,v_2)
  }
  \\
  \inferrule
  {
    \inferrule
    {
     \strut
    }
    {
      \kwfst{\kwpair{v_1}{v_2}}
      \red
      v_1
    }
    \\
    \inferrule
    {
     \strut
    }
    {
      \kwsnd{\kwpair{v_1}{v_2}}
      \red
      v_2
    }
  }
  {
    \kwsnd{\kwpair{v_1}{v_2}} 
    + 
    \kwfst{\kwpair{v_1}{v_2}}
    \red 
    v_3
  }    
}
{
\kwlet
{x}
{e}
{\kwsnd{x} + \kwfst{x}}
\red
v_3
}
\end{array}
\]
}}

\nocaptionrule
\caption{A derivation.}
\label{fig:example-let-sum}
\end{figure}


==> fig-example-let-swap.tex <==
\sethlcolor{SpringGreen}
\begin{figure}
\small
\fbox{\parbox{\columnwidth}{
\[
\begin{array}{c}
\inferrule*
{
  \inferrule*
  {
   1 \red 1
   \\
   \hlm{2 \red 2}
  }
  {
    \kwpair{1}{2}
    \red 
    \kwpair{1}{2}
  }
  \\
  \inferrule
  {
    \inferrule
    {
     \kwpair{1}{2} 
     \red 
     \kwpair{1}{2}
    }
    {
      \kwfst{\kwpair{1}{2}}
      \red
      1
    }
    \\
    \inferrule
    {
     \kwpair{1}{2} 
     \red 
     \kwpair{1}{2}
    }
    {
      \kwsnd{\kwpair{1}{2}}
      \red
      2
    }
  }
  {
    \kwpair{\kwsnd{\kwpair{1}{2}}}
           {\kwfst{\kwpair{1}{2}}}
    \red 
    \kwpair{2}{1}
  }    
}
{
\kwlet
{x}
{\kwpair{1}{2}}
{\kwpair{\kwsnd{x}}{\kwfst{x}}}
\red
\kwpair{2}{1}
}
\end{array}
\]
}}

\nocaptionrule
\caption{A derivation and a slice (highlighted).}
\label{fig:example-let-swap}
\end{figure}


==> fig-example-swap.tex <==
\sethlcolor{SpringGreen}
\begin{figure}
\small
\fbox{\parbox{\columnwidth}{
\[
\begin{array}{c}
\inferrule*
{
    \inferrule*
    {
     \inferrule*
     {
       a \red a \\ 
       \hlm{b \red b}
     }
     {
          \kwpair{a}{b} 
          \red 
          \kwpair{a}{b}
     }     
    }
    {
      \kwsnd{\kwpair{a}{b}}
      \red
      b
    }
    \\
    \inferrule*
    {
     \inferrule*
     {
       a \red a \\ 
       b \red b
     }
     {
          \kwpair{a}{b} 
          \red 
          \kwpair{a}{b}
     }     
    }
    {
      \kwfst{\kwpair{a}{b}}
      \red
      a
    }
}
{
\kwpair{\kwsnd{\kwpair{a}{b}}}{\kwfst{\kwpair{a}{b}}}
\red
\kwpair{b}{a}
}
\end{array}
\]
}}
%
\nocaptionrule
\caption{A derivation and a backward slice (highlighted).}
\label{fig:example-swap}
\end{figure}


==> fig-nrc-recomputation.tex <==
\begin{figure*}[tb]
\fbox{$\gamma, T \trrun v,T'$}
\vspace{-2ex}
\begin{smathpar}
\inferrule*{\strut}
{
\gamma,\tremp \trrun \tremp,\tremp
}
%
\and
%
\inferrule*{\strut
}{
\gamma, \kwc \trrun \kwc,\kwc
}
%
\and
\inferrule*{\gamma,T_1 \trrun \kwc_1,T_1'\\
\cdots\\
\gamma,T_n \trrun \kwc_n,T_n'
}{
\gamma,\kwf(T_1,\ldots,T_n) \trrun \hat{\kwf}(\kwc_1,\ldots,\kwc_n),\kwf(T_1',\ldots,T_n')
}
%
\and
\inferrule*{\strut
}{
\gamma,x \trrun \gamma(x),x
}
%
%
\and
%
\inferrule*{
\gamma,T_1 \trrun v_1,T_1'\\
\gamma[x\mapsto v_1],T_2 \trrun v_2,T_2'
}{
\gamma,\kwlet{x}{T_1}{T_2} \trrun v_2,\kwlet{x}{T_1'}{T_2'}
}
%
\and
%
\inferrule*{
\gamma,T_1 \trrun v_1,T_1\\
\cdots\\
\gamma,T_n \trrun v_n,T_n
}{
\gamma,\kwrec{A_1{:}T_1,\ldots,A_n{:}T_n} \trrun \kwrec{A_1{:}v_1,\ldots,A_n{:}v_n},\kwrec{A_1{:}T_1',\ldots,A_n{:}T_n}
}
%
\and
\inferrule*{
\gamma,T\trrun \kwrec{A_1{:}v_1,\ldots,A_n{:}v_n},T'
}{
\gamma,\kwfield{T}{A_i} \trrun v_i,\kwfield{T'}{A_i}
}
%
\and
\inferrule*{
\gamma,T \trrun \kwtrue,T' \\
\gamma,T_1 \trrun v_1,T_1'
}{
\gamma,\trifthen{T}{e_1}{e_2}{T_1} \trrun v_1,\trifthen{T'}{e_1}{e_2}{T_1'}
}
%
\and
\inferrule*{
\gamma,T \trrun \kwfalse,T' \\
\gamma,e_2\trrun v_2,T_2'
}{
\gamma,\trifthen{T}{e_1}{e_2}{T_1} \trrun v_2,\trifelse{T'}{e_1}{e_2}{T_2'}
}
%
\and
\inferrule*{
\gamma,T \trrun \kwtrue,T' \\
\gamma,e_1 \trrun v_1,T_1'
}{
\gamma,\trifelse{T}{e_1}{e_2}{T_2} \trrun v_1,\trifthen{T'}{e_1}{e_2}{T_1'}
}
%
\and
\inferrule*{
\gamma,T \trrun \kwfalse,T' \\
\gamma,T_2\trrun v_2,T_2'
}{
\gamma,\trifelse{T}{e_1}{e_2}{T_2} \trrun v_2,\trifelse{T'}{e_1}{e_2}{T_2'}
}%
\and
\inferrule*{
\gamma,T \trrun \tremp,T'
}{
\gamma,\trifelse{T}{e_1}{e_2}{T_2} \trrun v_2,\trifelse{T'}{e_1}{e_2}{\tremp}
}%
\and%
\inferrule*
{\strut}
{\gamma,\emptyset \trrun \emptyset,\emptyset}
%
\and
%
\inferrule*
{
\gamma,  T \trrun v,T'
}
{
\gamma, \trsets{T} \trrun \kwsets{\epsilon.v},\trsets{T'}
}
%
\and
%
\inferrule*
{
\gamma, T_1 \trrun v_1,T_1'
\\
\gamma, T_2 \trrun v_2,T_2'
\\
}
{
\gamma,\trsetu{T_1}{T_2} \trrun 1 \cdot v_1 \semu 2 \cdot v_2,\trsetu{T_1'}{T_2'}
}
%
\and
%
% \inferrule*
% {
% \gamma, T \trrun \kwset{\bindl{\lbl_1'}{v_1},\ldots,\bindl{\lbl_m'}{v_m}} 
% %\\
% %v = v_1\semu \ldots \semu v_n
% }
% {
% \gamma, \trflatten{T} \trrun v_1\semu \ldots \semu v_m
% }
%
\and
%
\inferrule*
{
\gamma,T \trrun \kwset{\bindl{\lbl_1}{v_1},\ldots,\bindl{\lbl_n}{v_n}} ,T'
%\\
%v = v_1\semplus \ldots \semplus v_n
}
{
\gamma, \trsetsum{T} \trrun v_1\semplus \ldots \semplus v_n,\trsetsum{T'}
}
%
\\
%
\inferrule*
{
\gamma,T \trrun v,T' \\ v = \emptyset
}
{
\gamma, \trsetise{T} \trrun \kwtrue,\trsetise{T'}
}
%
\and
%
\inferrule*
{
\gamma,T \trrun v,T' \\ v \not= \emptyset
}
{
\gamma, \trsetise{T} \trrun \kwfalse,\trsetise{T'}
}
%
\and
%
\inferrule*
{
\gamma, T \trrun v,T' \\
 \gamma,x\in v, \Theta,e' \trrun^* v',\Theta'
}
{
\gamma, \trcomp{e}{x}{T}{\Theta}
\trrun
v',\trcomp{e}{x}{T'}{\Theta'}
}
\end{smathpar}


\fbox{$\gamma,x\in v, \Theta,e \trrun^* v'$}
\vspace{-2ex}
\begin{smathpar}
\inferrule*
{
\strut
}
{
 \gamma,x\in \emptyset, \Theta,e \trrun^* \emptyset,\emptyset
}
%
\and
%
\inferrule*
{
\gamma,x\in v_1,\Theta,e \trrun^* v_1',\Theta_1'\\
\gamma,x\in v_2,\Theta,e \trrun^* v_2',\Theta_2'\\
}
{
\gamma,x\in v_1\semu v_2,\Theta,e \trrun^* v_1'\cup v_2',\Theta_1'\semu \Theta_2'\\
}
%
\and%
\inferrule*
{
 \lbl_i \in \dom(\Theta) \\
 \gamma[x\mapsto v_i],\Theta(\lbl_i) \trrun v_i',T' 
}
{
 \gamma,x\in \set{\lbl_i.v_i}, \Theta,e \trrun^* \lbl_i \cdot v_i',\{\lbl_i.T'\}
}
%
\and
%
\inferrule*
{
 \lbl_0 \notin \dom(\Theta) \\
 \gamma[x\mapsto v_0],e \red v_0' ,T'
}
{
  \gamma,x\in \set{\lbl_0.v_0}, \Theta,e \trrun^* \lbl_0\cdot v_0',\{\lbl_0.T'\}
}
\end{smathpar}
\caption{Trace recomputation.}
\label{fig:nrc-recomputation}
\end{figure*}


==> fig-nrc-trace.tex <==
\begin{figure}
\begin{sdisplaymath}
\begin{array}{@{}l@{\quad}r@{~~}c@{\quad}l}
\mbox{Traces} & 
T & \bnfdef & 
\ldots \bnfalt
\emptyset \bnfalt
\trsets{\lbl}{T} \bnfalt 
\trsetu{T_1}{T_2} \bnfalt
\trflatten{T} \bnfalt
%\\
%& & \bnfalt & 
\trsetsum{T} \bnfalt
\trsetise{T} 
\\
& & \bnfalt & 
\trsetcomp{\trbindl{l_1}{l_1'}{T_1'}, \ldots,
  \trbindl{l_n}{l_n'}{T_n'} }{T}{x}{e'} 
\end{array}
\end{sdisplaymath}
%\nocaptionrule
\caption{NRC: Traces}
\label{fig:nrc-trace-syntax}
\end{figure}


==> fig-path-ops.tex <==
\begin{figure}
\begin{mathfig}
\begin{array}{rcl}

\paths(\kwc) &=& \{\epsilon\}
\\
\paths((v_1,v_2)) &=& \{1\cdot p \mid p \in \paths(v_1)\}
\\
&\cup & \{2\cdot p \mid p \in \paths(v_2)\}
\\
\paths(\kwlam{x}{e}) &=& \{\epsilon\}
\\[2mm]
%

\atpath{v}{\pe} & = & v 
\\
\atpath{\kwpair{v_1}{v_2}}{\pcons{1}{p}} & = & \atpath{v_1}{p}
\\
\atpath{\kwpair{v_1}{v_2}}{\pcons{2}{p}} & = & \atpath{v_2}{p}
\\[2mm]
%
\mappath{v}{\pe} & = & v
\\
\mappath{\kwpair{v_1}{v_2}}{\pcons{1}{p}} & = & \kwpair{\mappath{v_1 }{p}}{\hole}
\\
\mappath{\kwpair{v_1}{v_2}}{\pcons{2}{p}} & = & \kwpair{\hole}{\mappath{v_2}{p}}
\end{array}
\end{mathfig}

\caption{Path operations,  \paths(v), \atpath{v}{p} and \mappath{v}{p}.}
\label{fig:path-ops}
\end{figure}


==> framework.tex <==
\section{A Framework for Provenance: Provenance Systems}

We develop a common framework for defining and comparing provenance
systems by establishing several key properties.  Intuitively, a
provenance system a language, where the dynamic semantics generates
some trace of the computation, which is then used by a provenance
function to answer provenance queries.  We define forward and backward
provenance functions as maps between the parts of the input to parts
of the output.  We measure the performance of a pro system by the time
it takes to construct the trace and answer provenance queries.


\subsection{Provenance Systems}


We define a {\em language} $\lang$ as a quadruple,
%
$\lang=(\lexps,\lvals,\ltrs,\leval)$
%
consisting of a set of expressions~\lexps, a set of values~\lvals such
that~$\lvals \subseteq \lexps$, a set of traces~\ltrs, and a big-step
evaluation relation~\leval.  The expressions can include a set of
variables \lvars.
%
We use $e$ and variants to denote expressions, $v$ and variants to
denote values, $x,y$ and variants to denote variables, and $T$ and
variants to denote traces.
%
The evaluation relation maps an expression to a value and a trace,
i.e., $e \leval v, T$.  Throughout, we assume that expressions can be
assigned a unique parse tree, i.e., they are derived from an abstract
syntax.  As usual, we do not distinguish between an expression and its
parse tree and use the same symbol to denote both.
 
Let~\lbls be an unspecified set of {\em labels}.  A {\em labeled
  expression} is an expression all of whose subexpressions are labeled
with a unique label (over all sub-expressions) in \lbls.  Intuitively,
labels mark the nodes of the of the parse tree of an expression; each
label~\lbl defines the subexpression rooted at the node marked
with~\lbl.
%
%
We leave the syntax of labeled expressions unspecified.  Instead, we
rely on several relations for operating on labeled expressions.  The
function~$\lblsOf{e}$ maps an expression~$e$ to a set of labels.
%
The function~$\expAt{e}{\lbl}$ maps an expression~$e$ and a
label~$\lbl$ to the subexpression of~$e$ rooted at~$\lbl$.
%
For $\lbl_1,\lbl_2 \in \lblsOf{e}$, we say that $\lbl_1$ is an
ancestor of $\lbl_2$, written $\ancst{\lbl_1}{\lbl_2}{e}$, if $\lbl_1$
is an ancestor of $\lbl_2$ in $e$, i.e., $e[\lbl_2]$ is a
sub-expression of $e[\lbl_1]$ or $\lbl_2 \in \lblsOf{e[\lbl_1]}$.
%
We use the notation $\sub{\hole}{\lbl_1, \ldots, \lbl_n}{e}$ to denote
the expression obtained by substituting $\hole$ for the subexpressions
of $e$ at $\lbl_1, \ldots, \lbl_n$.  We refer to a language~\lang
whose labels are drawn from a set of labels~\lbls as a {\em labeled
  language}, written~$\lang_\lbls$.


\begin{definition}[Provenance System]
Let $\lang_\lbls = (\lexps, \lvals, \ltrs, \leval)$ be a labeled
language with label set \lbls.
%
A provenance system \ps{\lang_\lbls}{\pfunf}{\pfunb}{\treval} for
\lang is a triple consisting of the language, a forward provenance
and/or a backward provenance function $\pfunf,\pfunb: \lbls \times
\ltrs \ra \powerset{\lbls}$ mapping a label and a trace to a set of
labels, and an evaluation relation~$\treval \subseteq \ltrs \times
\lvals$ for traces.
\end{definition}
%
When a provenance system has both a forward and a backward provenance
function, \pfunf, and \pfunb (respectively), we say that they are {\em
  consistent} if for any $e \leval v, T$,
\[
\pfunb(\lbl) = 
\{
\lbl' ~|~ \lbl' \in \lblsOf{e} \land \lbl \in \pfunf(\lbl')
\}.
\]
%


\subsection{Semantic Properties of Provenance}
We identify two semantics properties of provenance systems, dependency
correctness and accuracy, and introduce quantities for measuring the
performance of provenance systems.
%
To define the semantics properties, we only consider forward
provenance functions, because forward and backward provenance
functions are derivable from each other.


We start by dependency correctness. Intuitively, we say that a
provenance system is dependency correct if its forward provenance
function identifies all the parts of the output that depends on an
input label correctly, i.e., if we change the input label, then only
the parts of the output identified by the forward provenance function
will be affected.  
%
\begin{definition}[Dependency Correctness]
We say that provenance system
\ps{\lang_\lbls}{\pfunf}{\cdot}{\treval}, where the $\lang_\lbls =
(\lexps,\lvals,\ltrs,\leval)$ is dependency correct if the following
conditions hold for any $e, e' \in \lexps$.
%
If $e \leval v, T$, and $[\hole/\{\lbl\}]~e = [\hole/\{\lbl\}]~e'$ for
some $\lbl \in \lbls$ and $e' \leval v', \_$, and $\pfunf(\lbl,T) = L$
($L \subseteq \lbls$), then $[\hole/L]v = [\hole/L]v'$.
\end{definition}
%

Dependency correctness is a critical property that provenance
functions must satisfy.  By itself, however, it is not enough to
guarantee that the provenance function is indeed interesting.  For
example, the trivial provenance function, $\pfun_0(\cdots) = \lbls$
that claims dependence between any part of the input expression and
all parts of the output is dependency correct.  It is therefore
important to consider the accuracy of provenance functions.  

In developing the notion of accuracy, it turns out to be often helpful
to close forward provenance functions under descendant relation by
forcing all subexpression depend on the same label that their
ancestors depend on.
%
We say that a provenance function~$\phi$ is {\em closed} if
it is closed under the descendant relation, i.e., for any
expression~$e$ such that~$e \leval v, T$, and~$\phi(\lbl,T) = L$
if~$\lbl_v \in L$ and~$\ancst{\lbl_v}{\lbl_v'}{v}$ then~$\lbl_v' \in
L$.
%
We call a provenance system closed if its provenance function is
closed.  We obtain the closure of a provenance system $\pins$, written
$\closure{\pins}$, by replacing its provenance function $\phi$ with
its closure.  Note that computing the closure of a provenance function
(system) is straightforward in linear time in the size of the
resulting value.

\begin{theorem}[Closure Preserves Dependency Correctness]
\label{thm:closure-vs-dc}
If a provenance system $\pins =
\ps{\lang_\lbls}{\pfunf}{\cdot}{\treval}$ is dependency correct, then
its closure $\closure{\pins}$ is dependency correct. Conversely, if
$\pins$ is not dependency correct, then its closure $\closure{\pins}$
is not.
\end{theorem}
\begin{proof}
\todo{Should not be too difficult.}
\end{proof}
%
\thmref{closure-vs-dc} states that closure operation does not
contribute to the dependency correctness of the system.  Closing a
provenance system simply adds redundant information.  


We say that a forward provenance function is more accurate than
another if it identifies more accurate dependencies, i.e., the parts
of the output value that it identifies as dependent on an input label
are smaller subexpressions. 
%
\begin{definition}[Accuracy]
Let $\pins_1 = \ps{\lang_\lbls}{\phi_1}{\cdot}{\treval}$ $\pins_2 =
\ps{\lang_\lbls}{\phi_2}{\cdot}{\treval}$ be two provenance systems
for the the language $\lang_\lbls = (\lexps,\lvals,\ltrs,\leval)$ that
differ only in their provenance function.
%
We say that $\phi_1$ ($\phi_2$) is less (more) accurate than $\phi_2$
($\phi_1$), written $\phi_1 \lac \phi_2$ if any expression $e \in
\lexps$ and any evaluation $e \leval v, T$, it holds that for any
$\lbl_0 \in \lblsOf{e}$, and $\lbl_1 \in \phi_1(l,T)$, there exists
$\lbl_2 \in \phi_2(l_0,T)$ such that $\ancst{\lbl_1}{\lbl_2}{v}$.
\end{definition}


%
We now show that the accuracy ordering defines a quasiorder.
%
\begin{lemma}
The relation $\gac$ is reflexive and transitive, but not
antisymmetric.
\end{lemma}
\begin{proof}
Reflexivity relies on the reflexivity of the ancestor relationship
between labels of a value, i.e., for any label $\lbl \in \lblsOf{e}$,
$\ancst{\lbl}{\lbl}{e}$. To prove reflexivity, we map the labels of
one provenance function to themselves in the other suffices.

Transitivity relies on the transitivity of the ancestor relationship
between labels, i.e., for any $\lbl_1,\lbl_2,\lbl_2 \in \lblsOf{e}$,
if $\ancst{\lbl_1}{\lbl_2}{e}$ and $\ancst{\lbl_2}{\lbl_2}{e}$ then
$\ancst{\lbl_1}{\lbl_3}{e}$. 

Antisymmetry requires that if $\phi_1 \gac \phi_2$ and $\phi_2 \gac
\phi_1$ then $\phi_1 = \phi_2$.  The relation $\gac$ is not
antisymmetric.  For example, consider the labels $\lbl_1$ and $\lbl_2$
such that $\ancst{\lbl_1}{\lbl_2}{\cdot}$ in some unspecified result
value and 
%
$\phi_1 = \{(\lbl_0,\lbl_1)\}$ and 
%
$\phi_2 = \{(\lbl_0,\lbl_1),(\lbl_0,\lbl_2)\}$.
%
We have $\phi_1 \gac \phi_2$, because $\ancst{\lbl_1}{\lbl_1}{\cdot}$.
We have $\phi_2 \gac \phi_1$, because $\ancst{\lbl_1}{\lbl_2}{\cdot}$.
\end{proof}

We write $F_1 \eac F_2$ to indicate $F_1 \gac F_2$ and $F_2 \gac
F_1$.  

Since the accuracy ordering is a quasiorder, we can compare different
provenance functions.  But how can we determine their ordering?  We
prove, for this purpose, that we can use familiar subset comparisons
on the closures of provenance functions.
%
\begin{theorem}
\label{prop:closures}
Let $\pfun_1$ and $\pfun_2$ be provenance function for the same
language $\lang=(\lexps,\lvals,\ltrs,\leval)$.  The following hold:
\begin{eqnarray}
\pfun_1 \gac \pfun_2 &\iff& \pfun_1 \subseteq
\closure{\pfun_2}\\ 
%
\pfun_1 \gac \pfun_2 &\iff& \closure{\pfun_1} \subseteq
\closure{\pfun_2} \\
%
\pfun_1 \eac \pfun_2 &\iff& \closure{\pfun_1} = \closure{\pfun_2} \\
%
\pfun_1 \eac \pfun_2 &\iff& \closure{\pfun_1} \eac \closure{\pfun_2}
\end{eqnarray}
\end{theorem}
\begin{proof}
Suppose that $\pfun_1 \gac \pfun_2$.  We know that for any value $v$
and trace $t$ of \lang such that $\lbl_v' = \pfun_2(\lbl,T)$, we have
$\lbl_v = \pfun_1(\lbl,T)$ such that
$\ancst{\lbl_v'}{\lbl_v}{v}$. Thus $\lbl_v \in
\closure{\pfun_2}(\lbl,T)$. Thus $\pfun_1 \subseteq \closure{\pfun_2}$
and $\closure{\pfun_1} \subseteq \closure{\pfun_2}$.  The third
property follows easily because $\pfun_1 \eac \pfun_2$ if an only if
$\pfun_1 \gac \pfun_2$ (thus $\closure{\pfun_1} \subseteq
\closure{\pfun_2}$) and $\pfun_2 \gac \pfun_1$ (and $\closure{\pfun_1}
\subseteq \closure{\pfun_2}$).  The fourth property holds for any
equal provenance functions. 
\end{proof}


\begin{proposition}
Let $\pfun_1,\pfun_2,\pfun_3$ be provenance function for the same
language $\lang=(\lexps,\lvals,\ltrs,\leval)$.  We have
$\pmeet{\closure{\pfun_1}}{\closure{\pfun_2}} \gac \closure{\pfun_1}$
and if $\closure{\pfun_3} \gac \closure{\pfun_1}$ $\closure{\pfun_3}
\gac \closure{\pfun_1}$ and $\closure{\pfun_3} \gac \closure{\pfun_2}$
then $\closure{\pfun_3} \gac
\pmeet{\closure{\pfun_1}}{\closure{\pfun_2}}$.
\end{proposition}
\begin{proof}
For the first part, note that 
$\pmeet{\closure{\pfun_1}}{\closure{\pfun_2}} \subseteq
\closure{\pfun_1}$.  By \propref{closures}, it follows that
$\pmeet{\closure{\pfun_1}}{\closure{\pfun_2}} \gac
\closure{\pfun_1}$. 
%
For the second part, given $\closure{\pfun_3} \gac \closure{\pfun_1}$
and $\closure{\pfun_3} \gac \closure{\pfun_2}$ we know, by
\propref{closures}, that $\closure{\pfun_3} \subseteq
\closure{\pfun_1}$ and $\closure{\pfun_3} \subseteq
\closure{\pfun_2}$.  Thus it follows that $\closure{\pfun_3} \subseteq
\pmeet{\closure{\pfun_1}}{\closure{\pfun_2}}$ and thus
$\closure{\pfun_3} \gac \pmeet{\closure{\pfun_1}}{\closure{\pfun_2}}$
(again by \propref{closures}).
\end{proof}



\subsection{Algorithmic Properties of Provenance}
%
Let $\pins = \ps{\lang_\lbls}{\pfunf}{\pfunb}{\treval}$ where
$\lang_\lbls = (\lexps,\lvals,\ltrs,\leval)$ be a provenance system.
To measure the effectiveness of $\pins$, we define three measures:
overhead, time for a forward provenance query, and time for a backward
provenance query.  The {\em overhead} is the gap between $\leval$ and
a conventional evaluation function that mimics $\leval$ but does not
construct the trace.
%
The time for forward (backward) provenance query is the time for
computing a query, e.g., $\pfunf(\lbl, T)$ measured in the length of
the trace and/or the size of the output.  




==> lambda-completeness.tex <==
\subsection{Completeness}
\label{sec:lambda::completeness}

We define and prove a critical completeness property for traces and
trace slices.
%
Completeness for traces means that the trace has the same behavior as
the expression that generated it.
%
Completeness for slices means that the slice has the same behavior as
the original expression, restricting attention to the components of
the input or output that are of interest.
%
\paragraph{Types.}

To ensure that changes to the input are sensible, we employ a largely
straightforward type system for traces, expressions and values. Types
include base types and standard products $\tau \times \tau'$, and
function types $\tau \to \tau'$.  If $\Gamma$ is an environment
mapping variables to types and $\Delta$ maps labels to types, we write
$\Gamma;\Delta \ts \alpha : \tau$ to indicate that an expression,
trace, or value $\alpha$ has type $\tau$.  We often write just $\Delta
\ts \alpha : \tau$ when $\Gamma$ is empty, and we refer to $\alpha$ as
\emph{closed} in this case.  We say $\theta$ \emph{preserves} $\Delta$
provided that for all $\lbl:\tau \in \Delta$, we have $\Delta \ts
\theta(\lbl):\tau$.


%
\input{fig-lambda-trace-types}
%
%
The rules for trace typechecking, some of which are shown in
\figref{lambda-trace-types}, are largely straightforward. One minor
subtlety is that in the evaluation rules involving binding, we
introduce labeled values $\lbl.v$ into the expression or trace being
evaluated.  These labels are necessary to build traces, but they may
remain in the eventual result value, for example hidden inside a
$\lambda$-term.  At that point they are no longer useful and we use
the label removal operation $\abstr{v}{\lbl}$ to ensure that they do
not escape their scopes.


% \uremark{Do we have a type safety proof? If not, then I think we
%   should not even state anything here.  Proving type safety for a
%   big-step semantics is tricky. We can simply say we omit these
%   because they are well understood.  } 

Typechecking plays a small, but important role in the results, and we
will mention this role when needed, but not go into full detail.
Here, we only state the main substitution and type soundness
properties.
\begin{lemma}[Substitution]\label{lem:subst}
  ~  \begin{enumerate}
  \item Suppose $\alpha$ is a value or trace and $\beta$ is an
    expression, value or trace.  If $\Gamma;\Delta \ts \alpha : \tau$ and
    $\Gamma;\Delta,\lbl:\tau \ts \beta : \tau'$ then
    $\Gamma;\Delta,\lbl:\tau \ts \subst{\alpha}{x}{\beta} : \tau'$.
  \item If $\Delta \ts v : \tau$ and $\Gamma,x:\tau;\Delta \ts e :
    \tau'$ and $\lbl$ is fresh then $\Gamma;\Delta,\lbl:\tau \ts
    \subst{\lbl.v}{x}{e} : \tau$.
  \item If $\Delta,\lbl:\tau' \ts v : \tau$ then
    $\Delta \ts \abstr{v}{\lbl} : \tau$.
  \end{enumerate}
\end{lemma}
\begin{theorem}[Type Soundness]\label{thm:type-soundness}
~
\begin{enumerate}
  \item If $\Delta \ts e : \tau$ and $e \red v,T$ then
    $\Delta \ts v:\tau$ and $\Delta \ts T:\tau$.
  \item If $\Delta \ts T : \tau$ and $T \trrun v$ then $\Delta \ts v :
    \tau$.
  \end{enumerate}
\end{theorem}
\begin{proof}
  Most cases are straightforward, using a suitably generalized
  induction hypothesis.  We use \lemref{subst}(3) to deal with
  the label removal operations in the rules involving
  variable-binding.
\end{proof}

% \paragraph{Substitutions.}
% When stating the completeness theorems, we need to be able to change
% the input or the source data of an expression or a trace.  We achieve
% this by applying a substitution (\secref{lambda::dynamic}), written by
% $\theta$, mapping labels to values.


% \uremark{Does the proof need update now that application is different?}
% \james{Fixed}

\begin{lemma}[Replay substitution]\label{lem:replay-subst}
  If $T \trrun v$ then $\subst{\bindl{\lbl}{v}}{\lbl}{T'} \trrun v'$ if and
    only if $\subst{T}{\lbl}{T'} \trrun \abstr{v'}{\lbl}$.
\end{lemma}
\begin{theorem}[Completeness for Traces]\label{thm:completeness-trace}
  Let $e$ be a closed, well-typed expression such that $\Delta \ts e:
  \tau$ and $\theta$ be any label substitution preserving the types of
  labels in $\Delta$.
  % q
  If $e \red v,T$ and $\theta(e) \red v'$, then $\theta(T) \trrun v'$. 
  % 
  Furthermore, if $\theta$ is empty, then in the replay $\theta(T)
  \trrun v$, none of the expression-evaluation rules fire
  ($\dagger$1--3). 
\end{theorem}
\begin{proof}
  The proof is by induction on the structure of the derivation $e \red
  v, T$.  The most interesting cases are those in which the control
  flow of $\theta(T)$ differs from that of $\theta(e)$.  We present
  two representative cases, for conditionals and application.

If the derivations are of the form 
\[
    \inferrule*
    {
      e_1 \red \kwtrue, T_1
      \\
      e_2 \red v_2, T_2
    }
    {
      \strut
      \kwif{e_1}{e_2}{e_3} \red v_2, \trif{T_1}{T_2}{e_3}
    }
\]
\[
       \inferrule*
    {
      \theta(e_1) \red \kwfalse
      \\
      \theta(e_3) \red v_3'
    }
    {
      \theta(\kwif{e_1}{e_2}{e_3}) \red v_3'
    }
\]
then we can apply the induction hypothesis and rule ($\dagger1$) to derive:
\[
\inferrule*[Right=($\dagger$1)]
{
\theta(T_1) \trrun \kwfalse
\\
\theta(e_3) \red v_3'
}
{
\theta(\trif{T_1}{T_2}{e_3})
\trrun
v_3'
}
\]

Suppose the derivations are of the form:
\[    \small\inferrule*
    {
      e_1 \red \kwlam{x}{e}, T_1
      \\
      e_2 \red v_2,T_2
      \\
      \subst{\bindl{\lbl}{v_2}}{x}{e} \red v, T
      \\
      \mbox{fresh~\lbl}
    }
    {
      \kwapp{e_1}{e_2} \red \abstr{v}{\lbl}, \trapp{{x}.{e}}{T_1}{\lbl}{T_2}{\subst{T_2}{\lbl}{T}}
    }
\]
\[    \small\inferrule*
    {
      \theta(e_1) \red \kwlam{x}{e'}
      \\
      \theta(e_2) \red v_2'
      \\
      \subst{\bindl{\lbl}{v_2'}}{x}{e'} \red v'
      \\
      \mbox{fresh~\lbl}
    }
    {
      \theta(\kwapp{e_1}{e_2}) \red \abstr{v'}{\lbl}
    }
\]
Then by induction we immediately have $\theta(T_1) \trrun
\kwlam{x}{e'}$ and $\theta(T_2) \trrun v_2'$.  There are two cases.
If $\kwlam{x}{e'} = \kwlam{x}{\theta(e)}$, observe that
$\subst{\lbl.v_2'}{x}{e'} = \subst{\lbl.v_2'}{x}{\theta(e)} =
\theta'(\subst{\lbl.v_2}{x}{e})$ where $\theta'(\lbl) = v_2'$.  So, by
induction we have that $\theta'(T) \trrun v'$.
Moreover, using \lemref{replay-subst}, we also have that
$\theta(\subst{T_2}{\lbl}{T}) \trrun v'$ so can conclude:
\[
 \small\inferrule*
{
\theta(T_1) \trrun \kwlam{x}{\theta(e)}
\\
\theta(T[T_2/\lbl]) \trrun \abstr{v'}{\lbl}
}
{
\trapp{{x}.\theta({e})}{\theta(T_1)}{\lbl}{\theta(T_2)}{\theta(\subst{T_2}{\lbl}{T})} \trrun \abstr{v'}{\lbl}
}
\]

If $\lambda x.\theta(e) \neq \lambda x.e'$, then we can  use
rule $(\dagger 3)$ to conclude:
\[
 \small\inferrule*[Right=($\dagger$3)]
{
\theta(T_1) \trrun \kwlam{x}{e'}
\\
\lambda x.\theta(e) \neq \lambda x.e'
\\
\theta(T_2) \trrun v_2'
\\
\subst{\lbl.v_2'}{x}{e'} \red v'
}
{
\trapp{x.\theta(e)}{\theta(T_1)}{\lbl}{\theta(T_2)}{\theta(\subst{T_2}{\lbl}{T})} \trrun \abstr{v'}{\lbl}
}
\]

Finally, when the substitution is empty, none of the control-flow in
the trace changes, and thus we never need the re-evaluation rules
marked with $(\dagger)$.
\end{proof}
\begin{comment}
%\todo State this somewhere more prominent
Although fidelity is relatively easy to prove for this simple
language, it becomes more complicated for the Nested Relational
Calculus, as we shall see later.
\end{comment}

\begin{comment}
%\todo: something like this should be said in the intro. 
Of course, the original expression is also a complete
explanation.  So we might ask: What is the value-added of traces?  Why
not just keep the original expression?  We will return to these
questions later in discussing provenance extraction and trace slicing.
\end{comment}



\begin{theorem}[Completeness for Backward
  Slices]\label{thm:completeness-backward}
  Let $e$ be a closed, well-typed expression $\Delta \ts e: \tau$, and
  $T$, $v$ be the trace and the result for $e$, i.e., $e \red v, T$.
  Assume that $p, T \trbslice T_p$.
  % 
  For any label substitution $\theta$ preserving $\Delta$ and value
  $v$ such that $\theta(e) \red v$, there exists $v_p$ such that
  $\theta(T_p) \trrun v_p$ and $v \eqat{p} v_p$.
  % 
  Furthermore, if $\theta$ is empty, then none of the
  expression-evaluation rules ($\dagger$1--3) are needed to derive
  $\theta(T_p) \trrun v_p$.
\end{theorem}


For forward slices, the completeness theorem states that the forward
slice taken with respect to label \lbl can be used to update the
output under modifications or substitutions to only that label.
%
\begin{theorem}[Completeness for Forward Slices]\label{thm:completeness-forward}
  Let $e$ be a closed, well-typed expression $\Delta \ts e: \tau$, and
  $T$, $v$ be the trace and the result for $e$, i.e., $e \red v, T$.
  Let $T_\lbl$ be the forward-slice of $T$ with respect to a label
  $\lbl$, i.e. $\lbl, T \trbslice T_\lbl$.
  % 
  For any $v,v'$ such that $\lbl:\tau'\in\Delta$ and $\Delta \ts v :
  \tau'$ and $\subst{\lbl.v}{\lbl}{e}\red v'$, we have
  $\subst{\lbl.v}{\lbl}{T_\lbl} \trrun v'$.
%
  Furthermore, in the special case where $T \trrun v'$ then none of
  the expression-evaluation rules ($\dagger$1--3) are needed to derive
  $T_\lbl \trrun v'$.
\end{theorem}

\begin{comment}
%These are from the old write up.
%

\begin{definition}
  Suppose $T \trrun v_0$ and $\lbl$ is a free label in $T$. A
  \emph{forward slice} of $T$ with respect to $l$ is a subtrace $T'
  \trsub T$ such that for any values $v,v'$, if $\subst{v'}{l}{T} \trrun
  v$ then $\subst{v'}{l}{T'} \trrun v$.
\end{definition}
Again, we omit side-conditions concerning types. 

\begin{theorem}
  Suppose $T \trrun v$, where $T$ is a fully-cached expression. Let
  $\lbl$ be a label in $T$, and suppose $\lbl,T \trslice T'$.  Then
  $T'$ is a correct forward slice of $T$ with respect to $\lbl$.
\end{theorem}

\end{comment}



% LocalWords:  typechecking subst subtrace


==> lambda-slicing.tex <==
\subsection{Trace Slicing}
\label{sec:lambda-slicing}
\label{sec:lambda::slicing}


Provenance information often requires focusing on components of the
source of output data.  We may want to answer backward provenance
queries showing how some output part was computed or forward
provenance queries showing how some input part was used.
%
In this section, we describe techniques for computing {\em backward}
and {\em forward} slices for collecting provenance information for
backward and forward queries.  First, though, we introduce technical
machinery for using paths to address parts of values.


\paragraph{Paths and Equivalence.} 

%\input{fig-lambda-path-example}
\input{fig-path-ops}

Provenance requires referring to different parts of the source or or
output data.  To facilitate this, we use {\em paths}.  Informally,
starting at the root of a value, a path in the value leads to a
subexpression of the value.
%
Formally, we define a \emph{path} as a sequence of numbers, written
$[i \cdot j \cdot ...]$ and write $\pe$ for the empty path or
sequence, and $\pcons{i}{p}$ for the path whose first element is $i$
and whose tail is $p$.
%

We define several operations on paths and values: {\em paths}, {\em
  at-path} and {\em map-path}, whose definitions are shown in
\figref{path-ops}.
%
We define the \emph{set of paths} of a value $v$, written $\paths(v)$
as all the valid paths in $v$. 
%
We informally say that a path $p$ is in $v$ if $p \in \paths(v)$.
%
Given a path $p \in \paths (v)$, we write $\atpath{v}{p}$ (at-path) to
denote the sub-value of $v$ defined by the path $p$, and write
$\mappath{v}{p}$ (map-path) to denote the specialization of $v$ with
holes to map the path $p$.

As an example, % \figref{lambda::path-example} shows the structure of
consider the value $v =
\kwpair{\kwpair{\kwpair{1}{2}}{3}}{\kwpair{4}{5}}$ and its path set;
each subvalue is labeled by its path.
%
We have $\atpath{v}{[2]} = \kwpair{4}{5}$ and $\mappath{v}{[2]} =
\kwpair{\hole}{\kwpair{4}{5}}$, and 
%
$\atpath{v}{[1 \cdot 1 \cdot 2]} = 2$ 
%
and 
%
$\mappath{v}{[1 \cdot 1 \cdot 2]} =
\kwpair{\kwpair{\kwpair{\hole}{2}}{\hole}}{\hole}$.  Note that the
map-path operation preserves the skeleton of the path, i.e., for any
$p \in \paths(v)$, $\atpath{v}{p} = \atpath{(\mappath{v}{p})}{p}$.

Consider values $v_1$ and $v_2$ and a path $p$ such that $p \in
\paths(v_1)$ and $p \in \paths(v_2)$.  We say that values $v_1$ and
$v_2$ are {\em equal at $p$}, written $v_1 \eqat{p} v_2$, if
$\atpath{v_1}{p} = \atpath{v_2}{p}$ (or $\mappath{v_1}{p} =
\mappath{v_2}{p}$). 
%
For example, $\kwpair{1}{2} \eqat{[1]} \kwpair{1}{42}$ but
$\kwpair{1}{2} \not\eqat{[2]} \kwpair{1}{0}$.


\paragraph{Backward Slicing.}
%
\figref{lambda-back-slice} shows the rules for backward slicing.  We
define a judgment $p, T \trbslice T'$ that slices trace $T$ with
respect to a path $p$ to yield the slice $T'$, which itself is a
trace.
%
The rules can be viewed as traversing the trace backwards, looking for
parts of $T$ that contribute to the output at path $p$ and collecting
them while replacing the parts that do not contribute with a \hole. 

\input{fig-lambda-back-slice}


%
When slicing, we compute the slice of a subtrace of the given trace
with respect to an empty path, \pe, when the value computed by the
subtrace fully contributes to the result.  
%
%
Slicing the empty trace returns the empty trace.  The rules for labeled
values and cached values use the operation $\mappath{v}{p}$ to discard
parts of $v$ irrelevant to $p$.
%
Slicing a constant yields the constant.  To slice a pair with respect
to \pe, we slice the components with respect to \pe.  To slice a pair
with respect to a non-empty path, we slice the component specified by
the head of the path, retain the sliced trace, and replace the other
with a hole; this throws away the component that does not contribute
to the part of the result at the path. 
%
The rules for conditionals slice into the test (with \pe, because the
result of the conditional matters) and the taken branch with path $p$,
but do not examine the non-taken branch.
%
For let-bindings, we substitute the first $T_1$ into the body $T_2$
for the specified label and then slice.  This enables slicing $T_1$
for each use.
%
For application traces, we slice the first and the second part of the
application with an empty path, because their results may potentially
contribute to the evaluation (by determining the $\lambda$-abstraction
and the argument), but slice the body with respect to the specified
path $p$.


\paragraph{Forward slicing.}

Forward slicing aids in understanding how a single part of the input
influences the output.  We define an algorithm for forward slicing
with respect to $\lbl$ using a judgment $\lbl,T \trfslice T'$.  A
forward slice is an executable subtrace that correctly recomputes the
output when $\lbl$ is updated, holding all other input labels fixed.

\input{fig-lambda-forward-slice}


% \begin{definition}
%   Suppose $T \trrun v_0$ and $\lbl$ is a free label in $T$. A
%   \emph{forward slice} of $T$ with respect to $l$ is a subtrace $T'
%   \trsub T$ such that for any values $v,v'$, if $\subst{v'}{l}{T} \trrun
%   v$ then $\subst{v'}{l}{T'} \trrun v$.
% \end{definition}
% Again, we omit side-conditions concerning types. 

We give an algorithm for forward slicing in
Figure~\ref{fig:lambda-forward-slice}.  The basic idea is to traverse
a \emph{fully-cached} trace looking for occurrences of the label
$\lbl$.  By this we mean a trace that alternates between the cache
form $\trcache{T}{v}$ and the other syntactic forms.  This ensures
that we can erase parts of $T$ yet still recompute the full output by
using the cached values.  Once we determine that part of a trace
$\trcache{T}{v}$ does not depend on $\lbl$ (e.g., because it has no
free occurrences) we can replace that part with the subtrace
$\trcache{\tremp}{v}$.  We include many rules that bubble subtraces
that do not depend on $\lbl$ up through the trace.  We omit a number
of straightforward rules.  Effectively, this simple forward slicing
algorithm deletes parts of $T$ that do not mention $\lbl$.


% \begin{theorem}
%   Suppose $T \trrun v$, where $T$ is a fully-cached expression. Let
%   $\lbl$ be a label in $T$, and suppose $\lbl,T \trslice T'$.  Then
%   $T'$ is a correct forward slice of $T$ with respect to $\lbl$.
% \end{theorem}








% LocalWords:  subexpression subvalue subtrace subtraces


==> paths.tex <==
\begin{figure*}
\begin{verbatim}
datatype exp = Var of string 
             | Num of int
             | Pair of exp * exp
             | Fst of exp
             | Snd of exp
             | Let of string * exp * exp

datatype 'a tree = Node of 'a * 'a tree list

datatype trace = (exp * exp) tree

(* val subst : exp * string * exp -> exp *)
(* Non capture avoiding *)
  fun subst (Var y,x,e)          = if x = y then e else Var y
    | subst (Pair(e1,e2),x,e)    = Pair(subst( e1, x,e), subst (e2, x, e))
    | subst (Fst e',x,e)         = Fst(subst( e', x, e))
    | subst (Snd e',x,e)         = Snd(subst( e', x, e))
    | subst (Num i,x,e)          = Num i
    | subst (Let(y,e1,e2),x,e)   = Let(y,subst(e1,x,e), subst(e2,x,e))
  
(* val trace : exp -> exp * trace *)

fun trace (e as Num i) = (e, Node((e, e),[]))
    | trace (e as Pair(e1,e2)) = 
      let val (v1,t1) = trace e1
          val (v2,t2) = trace e2 
          val v = Pair(v1,v2)
      in (v,Node((e,v),[t1,t2]))
      end
    | trace (e as Fst(e')) = 
      let val (Pair(v,_),t) = trace e'
      in (v,Node((e,v),[t]))
      end
    | trace (e as Snd(e')) = 
      let val (Pair(_,v),t) = trace e'
      in (v,Node((e,v),[t]))
      end
    | trace (e as Let(x,e1,e2)) = 
      let val (v1,t1) = trace e1
          val (v2,t2) = trace (subst(e2,x,v1))
      in (v2,Node((e,v2),[t1,t2]))
      end
\end{verbatim}
\caption{Naive traces for let-pair language}
\end{figure*}

\begin{figure*}
\begin{verbatim}
type path = int list

(* val lookup : exp * path -> exp *)

  fun lookup (exp,[])            = exp
    | lookup (Pair(e1,e2),1::p)  = lookup(e1,p)
    | lookup (Pair(e1,e2),2::p)  = lookup(e2,p)
    | lookup (Fst(e),1::p)       = lookup(e,p)
    | lookup (Snd(e),1::p)       = lookup(e,p)
    | lookup (Let(x,e1,e2),1::p) = lookup(e1,p)
    | lookup (Let(x,e1,e2),2::p) = lookup(e2,p)

(* val pcons : step * path option -> path option *)


  fun pcons (s,NONE) = NONE
    | pcons (s,SOME p) = SOME (s::p)

(* val pmatch : exp * string * path -> path option *)

  fun pmatch (Var y, x, p)          = if x = y then SOME p else NONE
    | pmatch (Num i, x, p)          = NONE
    | pmatch (Pair(e1,e2),x,1::p)   = pmatch(e1,x,p)
    | pmatch (Pair(e1,e2),x,2::p)   = pmatch(e2,x,p)
    | pmatch (Fst(e),x,1::p)        = pmatch(e,x,p)
    | pmatch (Snd(e),x,1::p)        = pmatch(e,x,p)
    | pmatch (Let(y,e1,e2),x,1::p)  = pmatch(e1,x,p)
    | pmatch (Let(y,e1,e2),x,2::p)  = if x = y then NONE else pmatch(e2,x,p)
    | pmatch (_,_,_) = NONE
            \end{verbatim}
\caption{Paths and some basic path operations} 
\end{figure*}

\begin{figure*}
\begin{verbatim}
(* val whr : trace * path -> path option *)

  fun whr (Node((Num i,v),        []),      [])   = SOME []
    | whr (Node((Pair(e1,e2),v),  [T1,T2]), [])   = SOME []
    | whr (Node((Pair(e1,e2),v),  [T1,T2]), 1::p) = pcons(1,whr(T1,p))
    | whr (Node((Pair(e1,e2),v),  [T1,T2]), 2::p) = pcons(2,whr(T2,p))
    | whr (Node((Fst(e),v),       [T]),     p)    = pcons(1,whr(T,1::p))
    | whr (Node((Snd(e),v),       [T]),     p)    = pcons(1,whr(T,2::p))
    | whr (Node((Let(x,e1,e2),v), [T1,T2]), p)    = 
      (case whr(T2,p) 
        of NONE => NONE
         | SOME q => 
           case pmatch(e2,x,q) 
            of NONE => SOME (2::q)
             | SOME r => pcons (1,whr(T1,r)))
    | whr (_,                               _)    = NONE
\end{verbatim}
\caption{Extracting where-provenance from naive traces using paths}
\end{figure*}

\begin{figure*}
\begin{verbatim}
(* val lcons : int * path list -> path list *)

  fun lcons (i,ps) = List.map (fn p => i::p) ps

(* val dep : trace * path -> path list *)

  fun dep (Node((Num i,v),        []),      [])   = [[]]
    | dep (Node((Pair(e1,e2),v),  [T1,T2]), [])   = [[]]
    | dep (Node((Pair(e1,e2),v),  [T1,T2]), 1::p) = []::lcons(1,dep(T1,p))
    | dep (Node((Pair(e1,e2),v),  [T1,T2]), 2::p) = []::lcons(2,dep(T2,p))
    | dep (Node((Fst(e),v),       [T]),     p)    = []::lcons(1,dep(T,1::p))
    | dep (Node((Snd(e),v),       [T]),     p)    = []::lcons(1,dep(T,2::p))
    | dep (Node((Let(x,e1,e2),v), [T1,T2]), p)    = 
      []::List.concat (List.map (fn q => case pmatch(e2,x,q) 
                                          of NONE => [2::q]
                                           | SOME r => lcons (1,dep(T1,r)))
                                (dep(T2,p)))
    | dep (_,                               _)    = []
\end{verbatim}
\caption{Extracting ``dependency-provenance'' from naive traces using paths}
\end{figure*}

\begin{figure*}
\begin{verbatim}
signature TRACEABLE = 
  sig
    type exp
    type loc
    type trace
    val value  : exp -> bool
    val lookup : exp * loc -> exp
    val trace  : exp -> exp * trace
    val dep    : trace * loc -> loc list
    val whr    : trace * loc -> loc option
  end
\end{verbatim}
\caption{Interface}
\end{figure*}

==> ps.tex <==


\james{7/1: This will need to be rewritten to refer back to and
  generalize the development in the previous section.}

\section{Provenance Systems}

In this section, we set out some basic definitions and abstractions
that we believe provide a common foundation to all forms of provenance
we are aware of.

\paragraph{Standard and nonstandard semantics}
Many provenance techniques ``annotate'' expressions, values, or
computations with additional information.  Other techniques maintain
auxiliary ``trace'' information that is linked to the standard
expressions using some addressing scheme.  Both techniques can be
viewed as defining a ``nonstandard'' semantics of a language, perhaps
having certain additional formal or intuitive properties.  So we will
first define a class of

Let $\lexps$ be a \emph{language}, or set of (abstract) expressions.
We define an {\em interpretation} of $\lexps$ to be 

A \emph{semantics} is a triple,
%
$\lang=(\lexps,\lvals,\leval)$
%
consisting of a set of expressions \lexps, a set of values $\lvals$,
and a big-step evaluation relation $\leval \subseteq \lexps \times
\lvals \times \ltrs$.  The expressions can include a set of variables
\lvars.  Throughout we use $e$ and variants to denote expressions, $v$
and variants to denote values, $x,y$ and variants to denote variables.
We may refer to a semantics as being deterministic, total, etc. if the
evaluation relation is deterministic, total, etc.
%

Let $\lang,\lang'$ be languages.  An \emph{interpretation} $f : \lang
\to \lang'$ of $\lang$ in $\lang'$ is a pair of functions
$(f_1:\lexps_1 \to \lexps_2,f_2: \lvals_1 \to \lvals_2)$ satisfying $e
\leval v$ implies $f_1(e) \leval f_2(v)$ for all $e \in \lexps_1, v
\in \lvals_1$.  

Fix a language $\lang_0 = (\lexps_0,\lvals_0,\leval_0)$ where
$\lvals_0 \subseteq \lexps_0$, and call it a \emph{standard}
interpretation.  This is the language whose provenance we shall be
interested in studying.  A \emph{nonstandard semantics} of $\lang_0$
is a pair $(\lang,f : \lang \to \lang')$ such that both components of
$f$ are surjective.  

A \emph{traced semantics} is a structure $(\lexps, \lvals, \ltrs,
\leval)$ such that $(\lexps, \lvals \times \ltrs,\leval)$ is a
semantics.  Note that any nonstandard interpretation can be viewed as
a traced semantics simply by taking $\ltrs$ to be a singleton.  We
often write $e \leval v,T$ instead of $e \leval (v,T)$ when discussing
a traced semantics.  Naturally, we can identify a traced semantics
with the underlying semantics $(\lexps, \lvals \times \ltrs,\leval)$.
We can also ``forget'' the traces, yielding a semantics $(\lexps,
\lvals, \leval')$ where $e \leval v \iff \exists T. e \leval v,T$.


\paragraph{Locations and parts}
Another common feature of provenance techniques is that we wish to
refer to parts of values.  Often, parts can be addressed using paths;
sometimes it is preferable to introduce explicit labels to
address parts of data structures in a stable way.  Alternatively, we
may be interested in \emph{partial} expressions, values, or traces.

We wish to talk about locations or partial expressions in an abstract
way to remain general and avoid getting too bogged down in details of
syntax at this early stage.  

To deal with \emph{locations}, we rely on a {\em labeling scheme}
providing several relations for operating on labeled objects (i.e.,
expressions, values, or traces).  A labeling scheme is a structure
$(X,L,\lblsOf(-), \expAt{-}{-},-[-/-])$.  Here $X$ is the set of
objects, $L$ the set of locations.  The function $\lblsOf{x}$ maps an
object $x \in X$ to a set of locations in $x$.  The function $x[y/l]$
replaces the subobject of $x$ at location $l$ with $y$.
%
The function $\expAt{x}{\lbl}$ maps an object $x$ and a location
$\lbl$ to the subobject of $x$ rooted at $\lbl$.  

%
For $\lbl_1,\lbl_2 \in \lblsOf{x}$, we say that $\lbl_1$ is an
ancestor of $\lbl_2$, written $\ancst{\lbl_1}{\lbl_2}{e}$, if $\lbl_1$
is an ancestor of $\lbl_2$ in $e$, i.e., $e[\lbl_2]$ is a
sub-expression of $e[\lbl_1]$ or $\lbl_2 \in \lblsOf{e[\lbl_1]}$.
%

To deal with \emph{partial objects}, we consider a structure
$(X,\hole,\sqleq)$ where $\sqleq$ is a partial order (reflexive,
transitive, antisymmetric) with least element $\hole$.  



\begin{definition}[Provenance System]
Let $\lang_\lbls = (\lexps, \lvals, \ltrs, \leval)$ be a labeled
language with label set \lbls.
%
A provenance system \ps{\lang_\lbls}{\pfun}{\treval} for \lang is a triple
consisting of the language, a provenance function $\pfun: \lbls \times
\ltrs \ra \powerset{\lbls}$ mapping a label and a trace to a set of
labels, and an evaluation relation~$\treval$  for traces.
\end{definition}

We say that a provenance function $\phi$ is {\em closed} if it is
closed under the descendant relation.  More specifically, for any
expression $e$ such that $e \leval v, T$, and $\phi(\lbl,T) = L$ if
$\lbl_v \in L$ and $\ancst{\lbl_v}{\lbl_v'}{v}$ then $\lbl_v' \in L$.
%
We call a provenance system closed if its provenance function is
closed.  Note that we can obtain the closure of a provenance system
$\pins$, written $\closure{\pins}$, by replacing its provenance
function $\phi$ with its closure.  Note that computing the closure of
a provenance system by taking closure of its provenance function is
relatively straightforward (computation requires linear time in the
size of the resulting value).

\paragraph{TODO.}  We had some discussions about why the ``forward
    provenance'' is fully general, because it allows us to define the
    ``backward provenance'' also, provenance as a relation.  We want
        to articulate these here.

\subsection{Dependency Correctness}

\begin{definition}[Dependency Correctness]
We say that provenance system \ps{\lang_\lbls}{\pfun}{\treval}, where
the $\lang_\lbls = (\lexps,\lvals,\ltrs,\leval)$ is dependency correct
if the following conditions hold for any $e, e' \in \lexps$.
%
If $e \leval v, T$, and $[\hole/\{\lbl\}]~e = [\hole/\{\lbl\}]~e'$ for
some $\lbl \in \lbls$ and $e' \leval v', \_$, and $\pfun(l,T) = L$
($L \subseteq \lbls$), then $[\hole/L]v = [\hole/L]v'$.
\end{definition}

Note that the trivial provenance function, $\pfun_0(\cdots) = \lbls$
that claims dependence between any part of the input expression and
all parts of the output is dependency correct.  

\begin{theorem}[Closure Preserves Dependency Correctness]
\label{thm:closure-vs-dc}
If a provenance system $\pins = \ps{\lang_\lbls}{\pfun}{\treval}$ is
dependency correct, then its closure $\closure{\pins}$ is dependency
correct. Conversely, if $\pins$ is not dependency correct, then its
closure $\closure{\pins}$ is not. 
\end{theorem}
\begin{proof}
\todo{Should not be too difficult.}
\end{proof}

\thmref{closure-vs-dc} states that closure operation does not
contribute to the dependency correctness of the system.  Closing a
provenance system simply adds redundant information.


\subsection{Accuracy}


\begin{definition}[Accuracy]
Let $\pins_1 = \ps{\lang_\lbls}{\phi_1}{\treval}$ $\pins_2 =
\ps{\lang_\lbls}{\phi_2}{\treval}$ be two provenance systems for the
the language $\lang_\lbls = (\lexps,\lvals,\ltrs,\leval)$ that differ
only in their provenance function.
%
We say that $\phi_1$ ($\phi_2$) is less (more) accurate than $\phi_2$
($\phi_1$), written $\phi_1 \lac \phi_2$ if any expression $e \in
\lexps$ and any evaluation $e \leval v, T$, it holds that for any
$\lbl_0 \in \lblsOf{e}$, and $\lbl_1 \in \phi_1(\lbl_0,T)$, there exists
$\lbl_2 \in \phi_2(l_0,T)$ such that $\ancst{\lbl_1}{\lbl_2}{v}$.
\end{definition}

We show that with this definition, $\gac$ is a quasiorder:
\begin{proposition}
The relation $\gac$ is reflexive and transitive, but not antisymmetric
\end{proposition}
\begin{proof}
Reflexivity relies on the reflexivity of the ancestor relationship
between labels of a value, i.e., for any label $\lbl \in \lblsOf{e}$,
$\ancst{\lbl}{\lbl}{e}$. To prove reflexivity, we map the labels of
one provenance function to themselves in the other suffices.

Transitivity relies on the transitivity of the ancestor relationship
between labels, i.e., for any $\lbl_1,\lbl_2,\lbl_3 \in \lblsOf{e}$,
if $\ancst{\lbl_1}{\lbl_2}{e}$ and $\ancst{\lbl_2}{\lbl_3}{e}$ then
$\ancst{\lbl_1}{\lbl_3}{e}$. 

Antisymmetry requires that if $\phi_1 \gac \phi_2$ and $\phi_2 \gac
\phi_1$ then $\phi_1 = \phi_2$.  The relation $\gac$ is not
antisymmetric.  For example, consider the labels $\lbl_1$ and $\lbl_2$
such that $\ancst{\lbl_1}{\lbl_2}{\cdot}$ in some unspecified result
value and 
%
$\phi_1 = \{(\lbl_0,\lbl_1)\}$ and 
%
$\phi_2 = \{(\lbl_0,\lbl_1),(\lbl_0,\lbl_2)\}$.
%
We have $\phi_1 \gac \phi_2$, because $\ancst{\lbl_1}{\lbl_1}{\cdot}$.
We have $\phi_2 \gac \phi_1$, because $\ancst{\lbl_1}{\lbl_2}{\cdot}$.
\end{proof}

We write $F_1 \eac F_2$ to indicate $F_1 \gac F_2$ and $F_2 \gac
F_1$.  

\paragraph{TODO.}  What is the importance of having a quasiorder.

\paragraph{TODO.} Some motivation about why we care about the accuracy
and closure stuff. 



\begin{proposition}
\label{prop:closures}
Let $\pfun_1$ and $\pfun_2$ be provenance function for the same
language $\lang=(\lexps,\lvals,\ltrs,\leval)$.  The following hold:
\begin{eqnarray}
\pfun_1 \gac \pfun_2 &\iff& \pfun_1 \subseteq
\closure{\pfun_2}\\ 
%
\pfun_1 \gac \pfun_2 &\iff& \closure{\pfun_1} \subseteq
\closure{\pfun_2} \\
%
\pfun_1 \eac \pfun_2 &\iff& \closure{\pfun_1} = \closure{\pfun_2} \\
%
\pfun_1 \eac \pfun_2 &\iff& \closure{\pfun_1} \eac \closure{\pfun_2}
\end{eqnarray}
\end{proposition}
\begin{proof}
Suppose that $\pfun_1 \gac \pfun_2$.  We know that for any value $v$
and trace $t$ of \lang such that $\lbl_v' = \pfun_2(\lbl,T)$, we have
$\lbl_v = \pfun_1(\lbl,T)$ such that
$\ancst{\lbl_v'}{\lbl_v}{v}$. Thus $\lbl_v \in
\closure{\pfun_2}(\lbl,T)$. Thus $\pfun_1 \subseteq \closure{\pfun_2}$
and $\closure{\pfun_1} \subseteq \closure{\pfun_2}$.  The third
property follows easily because $\pfun_1 \eac \pfun_2$ if an only if
$\pfun_1 \gac \pfun_2$ (thus $\closure{\pfun_1} \subseteq
\closure{\pfun_2}$) and $\pfun_2 \gac \pfun_1$ (and $\closure{\pfun_1}
\subseteq \closure{\pfun_2}$).  The fourth property holds for any
equal provenance functions. 
\end{proof}


\begin{proposition}
Let $\pfun_1,\pfun_2,\pfun_3$ be provenance function for the same
language $\lang=(\lexps,\lvals,\ltrs,\leval)$.  We have
$\pmeet{\closure{\pfun_1}}{\closure{\pfun_2}} \gac \closure{\pfun_1}$
and if $\closure{\pfun_3} \gac \closure{\pfun_1}$ $\closure{\pfun_3}
\gac \closure{\pfun_1}$ and $\closure{\pfun_3} \gac \closure{\pfun_2}$
then $\closure{\pfun_3} \gac
\pmeet{\closure{\pfun_1}}{\closure{\pfun_2}}$.
\end{proposition}
\begin{proof}
For the first part, note that 
$\pmeet{\closure{\pfun_1}}{\closure{\pfun_2}} \subseteq
\closure{\pfun_1}$.  By \propref{closures}, it follows that
$\pmeet{\closure{\pfun_1}}{\closure{\pfun_2}} \gac
\closure{\pfun_1}$. 
%
For the second part, given $\closure{\pfun_3} \gac \closure{\pfun_1}$
and $\closure{\pfun_3} \gac \closure{\pfun_2}$ we know, by
\propref{closures}, that $\closure{\pfun_3} \subseteq
\closure{\pfun_1}$ and $\closure{\pfun_3} \subseteq
\closure{\pfun_2}$.  Thus it follows that $\closure{\pfun_3} \subseteq
\pmeet{\closure{\pfun_1}}{\closure{\pfun_2}}$ and thus
$\closure{\pfun_3} \gac \pmeet{\closure{\pfun_1}}{\closure{\pfun_2}}$
(again by \propref{closures}).
\end{proof}

\paragraph{TODO.} Talk about this significance/point of this. 




\subsection{Consistency and fidelity}

\begin{definition}
  [Consistency] A provenance system is consistent if for all $e,v,T$,
  $e \red v,T$ implies $T \trrun v$.
\end{definition}

\begin{definition}
  [Fidelity] A provenance system is faithful if for all
  $e,v,T,\theta$, $e \red v,T$ and $\theta e \red v'$ implies $\theta
  T \trrun v'$.
\end{definition}

\subsection{Subtraces and Consistency}

\paragraph{TODO.}  Note that we are considering typed languages where
traces and expressions are typed.  Also, we assume that there is a
definition of a subtrace (i.e. an ordering $\trsub$ on traces).


We will use 
% \begin{definition}[Consistent Subtrace]
% Let $e$ be a well typed expression, $ \ctxe \ts e :\tau$ and let $e
% \red v, T$ be an evaluation of $e$ yielding value $v$ and trace $T$.
% Let $p$ be a path in $v$ and $T' \trsub T$ be a well-typed subtrace of
% $T$ such that $ \ctxe \ts T' : \tau$.

% \begin{itemize}

% \item We say that $T'$ is (update) consistent with $e$ if for any $e'$
%   expression similar to $e$, i.e., $e \simx{L} e' : \tau$, where $L
%   \subseteq \lblsOf{e}$, $e'$ $e' \red v_0, \_$ then $e', T' \trrun
%   v_1$ and $\atpath{v_0}{p} = \atpath{v_1}{p}$.

% \item 
% We say that $T'$ partially (update) consistent with $e$ if for any
% $e'$ expression similar to $e$, i.e., $e \simx{L} e' : \tau$, where $L
% \subseteq \lblsOf{e}$, if $e' \red v_0, \_$ and $e', T' \trrun v_1$
% then either $v_1 = \bottom$ or $\atpath{v_0}{p} = \atpath{v_1}{p}$.

% \end{itemize}
% \end{definition}


\begin{definition}[Backward slices]
  Suppose $T \trrun v$ and $p \in v$.
  \begin{itemize}
  \item A \emph{consistent backwards slice} with respect to $p$ is a
    trace $T' \trsub T$ such that for some $v'$, we have $T' \trrun
    v'$ and $\atpath{v}{p} = \atpath{v'}{p}$.
  \item A \emph{faithful backwards slice} with respect to $p \in v$ is
    a trace $T' \trsub T$ such that for any $\theta$, $v_0$, $v_0'$,
    if $\theta T \trrun v_0$ then $\theta T' \trrun v_0'$ where   $\atpath{v_0}{p} = \atpath{v_0'}{p}$.
  \end{itemize}
\end{definition}

\begin{definition}[Forward slices]
  Suppose $T \trrun v$ and $l \in T$.
  \begin{itemize}
  \item A \emph{consistent forward slice} is a trace $T' \trsub T$
    such that if $T[\hole/l] \trrun v'$ then $T'[\hole/l] \trrun v'$.
  \item A \emph{faithful forward slice} is a trace $T' \trsub T$ such
    that for any $v_0$ such that $T[v_0/l] \trrun v'$ we also have
    $T'[v_0/l] \trrun v'$.
  \end{itemize}
\end{definition}


\subsection{Principles}


Which of the following do you agree should always hold?

\begin{enumerate}\item 
  $T \trsub T$
\item  $T_1 \trsub T_2$ and $T_2 \trsub T_1$ implies $T_1 = T_2$
\item 
 $T_1 \trsub T_2$ and $T_2 \trsub
  T_3$ implies $T_1 \trsub T_3$ 
\item $T_1 \trsub T_2$ implies that for any $\theta,v$, if $\theta T_1 \trrun
  v$ then there exists $v'$ with $v \trsub v'$ and $\theta T_2 \trrun
  v'$.  
\item If for any $\theta,v$, if $\theta T_1 \trrun v$ then there
  exists $v'$ with $v \trsub v'$ and $\theta T_2 \trrun v'$, then $T_1
  \trsub T_2$
  \item $T \trrun v$ and $T \trrun v'$ implies $v = v'$
\end{enumerate}
I believe that (1,3,4,6) hold currently (for the let-pair language).  (2) and (5) depend heavily on the definition of subtrace.

Similarly, I have some intuitions about trace slices.  A "notion of slicing" is a function $S$ that maps traces $T$ to sets of subtraces of $T$, satisfying the following:

\begin{enumerate}
  \item $T$ is always in $S(T)$ (hence, $S(T)$ is never empty.)  
  \item $\tremp$ is never in $S(T)$ (provided $T$ itself has no
    occurrences of $\tremp$)
  \item If $T_1 \trsub T_2 \trsub T$ and $T_1 \in S(T)$ then $T_2 \in
    S(T)$.  (that is, $S(T)$ is ``closed upwards'')
  \item If $T_1,T_2 \in S(T)$ then there exists $T' \in S(T)$
    satisfying $T' \trsub T_1$ and $T' \trsub T_2$ such that T' is
    also in $S(T)$.  (that is, $S(T)$ is "closed under intersection").
\end{enumerate}

Do these seem like good ``axioms''?  For any ``notion of slicing''
satisfying (a-c), we can see that there must exist ``minimal'' slices;
also, if (d) holds then there must be unique ``minimum'' slices
(possibly modulo equivalence if subtrace is only a quasiorder.)



==> recomputation.tex <==
\section{Recomputation}
\label{sec:recomputation}

Replay allows for recomputing the \emph{full} trace. However, we may
often wish to only recompute a part of the trace to see how a change
to the input affects a specific part of the output. The ``golden
trail'' feature requested by many scientific users is a typical
example: after running a complex computation, perhaps involving sweeps
over several parameters and using several fitness functions to
identify promising results, a scientist may wish to extract a subset
of the provenance trace that recomputes \emph{just} the five most
interesting results, to allow further inspection and validation.

There are a number of interesting challenges involved in developing such a feature, such as how to present the full provenance trace or its subsets to users effectively; here, however, we focus just on the technical issue of how to extract enough 

The slicing algorithms given already suffice to explain how the result
was computed, provided the input is similar enough to the original
input to preserve relevant control flow choices. In fact, the existing
backward slicing algorithm already captures enough information to
recompute the part of the output with respect to which the slice was
computed, if it still exists. However, before we can make this precise, we need to
generalize the replay semantics. Sliced traces cannot always be rerun
due to the presence of holes. Thus, we extend the replay semantics
with the following rules that permit replaying traces that contain
holes. Thus, we generalize replay to a \emph{recomputation} judgment $\rho,T \trrun p,T'$ that allows replaying a partial trace on a partial environment; the results
may also contain holes.  \figref{nrc-recomputation} defines this judgment.


\begin{theorem}
  If $\gamma,e \red v,T$ and $p,T \trbslice \rho,S$ where $v \sqleq p$ then for any $\rho'$, if $\rho',S \trrun p',S'$ and $p \sqleq p'$ then $p' \simat{p} v$.
\end{theorem}

First, we show that the recomputation semantics satisfies a generalization of fidelity for replay, that is, the trace $T'$ obtained by recomputing a trace on a changed environment is athe same as that obtained by computing from scratch:
\begin{theorem}
  If $\gamma,e \red v,T$ then $\gamma',e \red v',T'$ if and only if $\gamma,T \trrun v',T'$.
\end{theorem}


\input{fig-nrc-recomputation}


